An Appraisal Transition System for Event-driven Emotions in Agent-based Player Experience Testing

Player experience (PX) evaluation has become a field of interest in the game industry. Several manual PX techniques have been introduced to assist developers to understand and evaluate the experience of players in computer games. However, automated testing of player experience still needs to be addressed. An automated player experience testing framework would allow designers to evaluate the PX requirements in the early development stages without the necessity of participating human players. In this paper, we propose an automated player experience testing approach by suggesting a formal model of event-based emotions. In particular, we discuss an event-based transition system to formalize relevant emotions using Ortony, Clore, & Collins (OCC) theory of emotions. A working prototype of the model is integrated on top of Aplib, a tactical agent programming library, to create intelligent PX test agents, capable of appraising emotions in a 3D game case study. The results are graphically shown e.g. as heat maps. Emotion visualization of the test agent would ultimately help game designers in creating content that evokes a certain experience in players.

==> techcontent2_orig.tex <==
%\vspace{-6mm}
%=================================================
\section{Proof of Concept}\label{sec.UXresult}
%==================================================

We conducted our experiment on a game called Lab Recruits\footnote{\url{https://github.com/iv4xr-project/iv4xrDemo/tree/occDemoPrototype}} which we subject to the combination of \aplib \ and our implemented model of appraisal\footnote{\url{https://github.com/iv4xr-project/jocc}} to provide the proof of concept and show our early results in PX testing. %Our implemented formal model of appraisal  serves as a reference implementation because it is directly translated from the mathematical model that we introduced according to the OCC theory. \XCOMMENT{I think the remark about 'reference implementation' is less useful in the paper, since we don't use it in its role as reference. This was the setup in that Formalise paper.}
Lab Recruits is a 3D game developed in Unity which has different replayable levels. Each level is a laboratory building with a number of rooms containing interactable objects, such as button and non-interactable objects, such as desk and fire hazards.

Figure \ref{subfigfloorplan} shows the floor plan of the level exposed to PX testing using our approach. It consists of four buttons, three doors, and some fire hazards. The goal is for the player to escape the level by reaching the exit room circled in red. Access to this room is guarded by a closed 'final door'.
The level contains some rooms with a puzzle (yellow circle) that involves finding the buttons to open the final door and reopen the doors that in the process become closed to entrap the agent. Figure \ref{subfigsetup1} and \ref{subfigsetup2} show two provided setups with the different amount and locations of fire hazards. The agent will lose health points by passing each fire hazard.
These setups are examples of %\DROP{test scenarios provided by}
choices considered by designers, although being currently simple, as to which one would lead to better PX.

\begin{figure}[htbp]
    \begin{minipage}{0.5\textwidth}
    %\centering
        \subfloat[The floor plan of the level.]{\includegraphics[width=0.9\textwidth]{emas21/floorplan_.png} \label{subfigfloorplan}}
    \end{minipage}
    %\qquad
    \begin{minipage}{0.5\textwidth}
    \centering
    \subfloat[\centering Setup 1.]{{\includegraphics[width=0.5\textwidth]{setup1.png} } \label{subfigsetup1}}  
    \subfloat[\centering Setup 2.] {{\includegraphics[width=0.5\textwidth]{setup2.png} }\label{subfigsetup2}}%
    \end{minipage}
    \caption{The level under the PX test in Lab Recruits.}%
    \label{figtestlevel}%
\end{figure}

As mentioned in Section \ref{sec.model}, a developer sets needed inputs of the model such as the goal set, initial likelihood of each goal, the desirability of events for each goal, the threshold and decay rate of emotions in {\em Player Characterization}. A test agent is deployed, set with multiple goals, though here we will only discuss the most significant one, namely completing the level.
Initially, the agent is assumed to believe that the likelihood of achieving this goal is  0.5.
The agent is given a program so that it can automatically explore the level.
As the agent progresses, its belief on the likelihood 
of completing the level changes, depending on the number of opened door as well as remained closed doors. Opening each door is assumed to have a desirable consequence for the agent because it increases the chance of the agent to complete the level.

The timeline of triggered emotions in the agent with respect to the goal "completing the level" is shown in Figure \ref{figtimeline}, along with their intensity levels at each time. The agent initially experience some hope and fear due to the assumed initial belief that completing the game is possible, with the likelihood 0.5. %The initial emotional state of the agent depends on its mood which influences the degree of hope and fear the agent initially has.
In both setups, when the agent pushes the button that opens the first door (time=70\footnote{The system is event driven, so only events can change the likelihoods. All emotions decay until an event is perceived. However, we can add an event type to the system to decay the likelihoods when there is no event for some period of time to update the emotional state.}), the agent's hope regarding completing the game starts to increase.  It decays or gets re-stimulated according to the events  until time 120 when it is replaced by joy. The agent feels a level of satisfaction,  When completing the game.
Comparing two setups reveals something interesting. Fear shows a quite different trend in setup 2 (Figure \ref{subfigtimeline.2}). It is strongly stimulated multiple times during the execution, whereas the same emotion is rarely stimulated in setup 1, and when it happens, it happens with much less intensity (Figure \ref{subfigtimeline.1}), towards the end of the play, where it matters less.
Such comparison can be useful for designers e.g. to determine the amount, and placement, of hazards to induce certain degree of fear along with keeping the chance for satisfactory experience of accomplishing the goal. In our case, setup 1 is less likely to thrill the player, whereas setup 2 has a better balance of the quantity and placement of the fire, by generating fear, while still keeping the level survivable.
%\INSERT{SA: this paragraph needs to be changed, please ignore it for now, a little wrong explanation}
%\XCOMMENT{WP: discuss $\rightarrow$}


\begin{figure}[htbp]
    \centering
    \subfloat[\centering Setup  1]{{\includegraphics[width=5.6cm, height=3.9cm]{emas21/emoOverTime_data_goalQuestCompleted_setup1.png} } \label{subfigtimeline.1}}
    \qquad
    \subfloat[\centering Setup 2]  {{\includegraphics[width=5.6cm, height=3.9cm]{emas21/emoOverTime_data_goalQuestCompleted_setup2.png} }\label{subfigtimeline.2}}% 
    \caption{The emotions' timelines correspond two setups of the game level in Figure. \ref{figtestlevel}.\\
   \centering {\small  (threshold=0, decay rate=0.005)} }%
    \label{figtimeline}%
\end{figure}

 Figure \ref{figheatmap} shows some heat maps, providing spatial information of the agent's emotions in Setup 2. Comparing the outcomes of Figures \ref{subfigtimeline.2} and  \ref{subfiggeat.1} illustrates that the highest level of fear is experienced between time 65 to 75 when the agent is in a particular fire covered corridor (yellow in Figure \ref{subfiggeat.1}). Fire intensifies the agent's fear of failure, and moreover the agent has to walk this corridor several times. The most drastic decline in fear is when the agent is about to finish the level.
\begin{figure}[htbp]
    \centering
    \subfloat[\centering Negative emotions: yellow= high fear, Orange shades=low fear.]{{\includegraphics[width=5.6cm]{emas21/overlay_emoColdmap_setup2.png} } \label{subfiggeat.1}}
   \qquad
    \subfloat[\centering Positive emotions: Mahogany red=hope, Ruby red= joy, yellow= satisfaction.]  {{\includegraphics[width=5.6cm]{emas21/overlay_emoHeatmap_setup2.png}}\label{subfigheat.2}}% 
    \caption{ \centering The heat maps of triggered emotions in setup 2.
    % breaking lines with \\ inside a caption is problematical for latex :|. Using this trick:
    \hspace{\textwidth}
    Black=no emotion, white= walls (not walkable), gray=unexplored area.}
    \label{figheatmap}%
\end{figure}
As can be seen in  Figure \ref{subfigheat.2}, the agent feels a higher level of hope when progressing in solving the buttons-doors puzzle in the puzzle rooms. After pushing the button that corresponds to the final door and reopening the door of puzzle room to escape it, the agent becomes certain that passing the final door is achievable now. Thus, the hope suddenly is replaced by the joy for reaching the final door to complete the game. At the end, the agent feels satisfied when the achievement is confirmed.  
Having such information would help Lab Recruits designers to adjust the puzzles and fire hazards in such a way to induce certain emotions, at the right moments and the right places, which ultimately affect a certain aspect of player experience like enjoyment.
